Revisiting Client Puzzles for State Exhaustion Attacks Resilience

In this paper, we address the challenges facing the adoption of client puzzles as means to protect the TCP connection establishment channel from state exhaustion DDoS attacks. We model the problem of selecting the puzzle difficulties as a Stackelberg game with the server as the leader and the clients as the followers and obtain the equilibrium solution for the puzzle difficulty. We then present an implementation of client puzzles inside the TCP stack of the Linux 4.13.0 kernel. We evaluate the performance of our implementation and the obtained solution against a range of attacks through experiments on the DETER testbed. Our results show that client puzzles are effective at boosting the tolerance of the TCP handshake channel to state exhaustion DDoS attacks by rate limiting the flood rate of malicious attackers while allocating resources for legitimate clients. Our results illustrate the benefits that the servers and clients amass from the deployment of TCP client puzzles and incentivize their adoption as means to enhance tolerance to multi-vectored DDoS attacks

==> abstract.tex <==
%Recent years have witnessed an increase in the scale and complexity
%of distributed denial of service attacks, with targets ranging from
%ordinary services to essential Internet infrastructure. DDoS tolerance by expansion of 
%resources comes at a high cost for defenders while scalable attacks come at a much lower 
%costs. Client puzzles present a promising avenue to even the imbalance between the attack and 
%defense costs by requiring users, both benign and malicious, to present the target server with the solution of a cryptographic puzzle as `payment' for the requested resources. 

In this paper, we
target the challenges facing the adoption of client puzzles as means to protect
the TCP connection establishment channel from DDoS attacks. We model the problem of selecting
the puzzle difficulties as a Stackelberg game with the server as the leader and the users as the followers and obtain the equilibrium solution for the puzzle difficulty. 
We then present an implementation of client puzzles inside the 
TCP stack of the Linux 4.13.0 kernel. 
We evaluate the performance of our implementation and the obtained solution against a range of attacks through  experiments on the DETER testbed. Our results show that client
puzzles are effective at boosting the tolerance of the TCP handshake channel against 
DDoS attacks through rate limiting the flood rate of malicious attackers while guaranteeing service for legitimate clients. We believe our results illustrate the benefits that the servers and users amass from the deployment of TCP client puzzles and incentivize their adoption as means for DDoS tolerance. 


==> background.tex <==
In this work, we focus on DoS attacks targeting the consumption of critical target computational resources such as
memory or CPU. Malicious actors also target network resources by initiating network flooding and reflection attacks.
% Defense mechanisms aiming to protect the networking infrastructure can substantially differ from those developed to
% protect computational resources, but similarities still can be found. 
In what follows, we discuss the different
techniques proposed to thwart computational resources DoS attacks and their shortcomings and then focus on existing
client puzzles techniques.

%% traditional techniques
\subsection{Traditional Approaches}
Traditionally, DDoS defense techniques aimed to either {\em filter} bad traffic or to 
{\em authorize} users before allocating resources. 
Capability-based approaches~\cite{Xiaowei2008,Xiaowei2005,Parno2007}
aim to authorize users by the means of
cryptographic packet capabilities. Application servers issue capabilities
(typically exchanged during connection setup) and require the routers on the
path between the clients and the servers to enforce their usage.
Capabilities allow servers and routers to rate limit or blacklist users based
on their observed behavior; detected bots will have their packets dropped as
early as their gateway router.

Filtering approaches rely on their ability to 
differentiate between legitimate and attach traffic in the network~\cite{liu2008, liu2010}, 
at the receiver~\cite{mahajan2002}, or at the Internet Service Provider (ISP)~\cite{fayaz2015}. The malicious traffic is then 
either dropped at the routers or redirected to spefic parts of the protection mechanism for further
analysis. 

%% Need analysis of shortcomings of these approaches here!
Both filtering and authorization techniques suffer from several drawbacks. First, they require changes
to the core Internet routers along the paths between different endpoints. Additionally, some of the
techniques require cooperation between ISPs, which is hard to achieve without proper incentives or government mandates. 
Furthermore, a crucial requirement for such techniques to work is their ability to differentiate between malicious and benign traffic.
However, attackers often leverage IP spoofing, reflection attacks, and make use of very large botnets
(reaching up to millions of machines) of unsuspecting users as weapons for mounting DDoS attacks.
This, therefore, makes the process of detecting malicious traffic and IP addresses intractable.

%% Now need to talk about syn cookies
\subsection{SYN cookies}
SYN cookies present a stateless method to combat server resource DoS attacks, specifically targeted 
against SYN flooding attacks~\cite{lemon2002,cryptosyncookies}. SYN floods are attacks that target the three-way handshake of
TCP. Once a server receives a synchronize (SYN) packet froma potential client, it reserves a slot in 
its queue for this client. In a SYN flood, the attackers overwhelm the server with a flood of SYN packets
and occupy the entire TCP backlog. Once that happens, the server discards new connection requests thus 
hindering the new clients' connectivity and service availability. When SYN cookies are enabled, the server
encodes a new TCP connection's parameters as a cookie in the packet's initial sequence number, 
and refrains from allocating state for a new connection until the cookie is again received from the client
and validated. 

Although SYN cookies eliminate the key target of the SYN flood attack (the TCP backlog), 
they do not provide protection against large botnets. Attackers in control of a large number of 
zombie machines with valid (non-spoofed) IP addresses can overload the server's TCP accept
queue with valid TCP requests without addded effort. By only tackeling the problem on the server end, 
SYN cookies do not present a mechanism to strip the malicious actors from the ability to conduct DoS attacks and prevent legitimate 
users from obtaining service. Furthermore, it is not clear how SYN cookies can be generalized to server 
as DoS protection schemes for different types of server resource DoS attacks (e.g. attacks against TSL connection 
setup)~\cite{wang2003}.

\subsection{Client puzzles}
\begin{figure}
  \centering
  \resizebox{0.5\columnwidth}{!}{%
	\includegraphics{puzzle_protocol.pdf}
  }
  \caption{A sample puzzle protocol.\tochange{Add writings on the side}}
  \label{fig:protocol}
\end{figure}

% Client puzzles - briefly
Cryptographic client puzzles have been proposed to counter the main asymmetry in today's Internet: the clients can
request large server resources at relatively little costs. DDoS resistance using client puzzles is premised on the
observation that under attack, alleviating this asymmetry can be done by forcing clients to pay 
-- using computing power -- for the server resources that they are requesting. In the case of a TCP SYN request, a 
client demanding a spot in the server's TCP backlog and accept queue must present a solution to a cryptographic 
puzzle as proof of her need for the server's resources. Such an approach will effectively hinder malicious attackers' 
ability to occupy space in the server's memory at virtually no cost of their own. Furthermore, when attackers employ 
botnets comprised of millions of unsuspecting users, a sudden churn in the unsuspecting machine's processing
jobs can alert its user to the presence of malware. 

Client puzzles have been previously proposed as a mechanism to combat junk mail~\cite{dwork1993}, website
metering~\cite{franklin1997}, protecting the TCP SYN channel~\cite{juels1999,mcnevin2004,wang2003,feng2005}, 
protecting the TLS connection setup~\cite{dean2001,ietf-draft}, and protecting the capabilities-granting channel~\cite{Parno2007}.
Additionally, client puzzles are at the heart of the mining process of nowadays'
crypto-currencies~\cite{nakamoto2008,bonneau2015}. Figure~\ref{fig:protocol} illustrates how client puzzles can help in
protecting the TCP connection establishment channel. Upon receiving a SYN packet, the server computes a puzzle
challenge and sends it back to the client. At this time, the server does not commit any resources to the initiating
client. The client, after receiving the challenge, will employ its computational resources to solve the challenge and 
send the solution back to the server. If the solution is correct, the server then commits resources to the client and
resumes the standard TCP connection setup mechanism. Otherwise, the server drops the connection. Although this process
violates the standard TCP protocol, the challenge and its solution can be easily piggybacked on the SYN/ACK and the
following ACK packet as we discuss later on in the paper. 

Despite its promise, there are several challenges that face the adoption of client puzzles as an effective measure
of defense against resource exhaustion DoS attacks. First, there is a shortage of implementations that allow for the
comparison and the evaluation between different types of challenge creation and verification mechanisms.
Although the IETF has proposed a draft to include client puzzles as a protection mechanism against resource exhaustion 
attacks in the TLS connection setup channel, we are yet to find implementations of client puzzles in the commonly used
TSL packages such as OpenSSL. Second, an important advantage of client puzzles is the ability to increase the difficulty
of the challenges as the intensity of the attacks increases. However, there are no tangible and theoretically-backed 
recommendations for selecting the appropriate challenge difficulties. Finally, client puzzles introduce
the possibility of an attack against the puzzle verification mechanism. Since the server does not keep state after
sending the challenge packet, an attacker can flood the server with a false challenge solution and force it into
spending much of its computing resources cryptographically verifying the solutions. 
In this work, we address the first two problems and provide a discussion and future suggestions on tackling the
third. 
\suggestion{talk a bit about how we address them. Use ns3 simulation and linux kernel implementation 
for the first and game theory for the second.}


\remove{%
  To counter the shortcomings of the aforementioned techniques, researchers 
  proposed client puzzles as a stateless approach to combat DDoS attacks. 
  Client puzzles are cryptographic operations that servers can ask their clients
  to solve, and are considered as currency paid in exchange for bandwidth, 
  compute, or disk resources~\cite{}. The more resources a client requires the
  less priority their traffic obtains, and thus are forced to increase the
  difficulty of the puzzles they must solve. The key observation is that zombie
  machines would avoid solving difficult puzzle in order not to alert their
  benign users of any compromise. 
}

% So basically the problems are
%	- architecture level changes (such as capability routers)
%	- inter-ISP cooperation, usually faced with political and economic hurdles
% 	- putting too much burden on the client to authenticate theirselves when
% under attack, something that should not be handed off totally to the clients
%themselves. 
%%Such techniques usually require
%
\remove {%
  The techniques mentioned above suffer from several drawbacks. Capabilities
  require intrusive infrastructural support from Internet routers, a privilege
  not usually available, a virtue of the Internet's complexity, scale, and
  immense politics. 
  Puzzle based approaches push the burden of DDoS resistance onto the client
  machines, many of which might not possess or might not be willing to use the
  needed computational resources for solving the puzzles. Additionally, many of
  the today's Internet of Things (IoT) devices are idle for significant periods
  of time, allowing attackers to make use of idle times to compute the puzzles
  undetected. 
  Furthermore, a common trend is all DDoS defense approaches is their reliance on
  distinguishing benign clients from malicious bots, a detection process often
  time-consuming, 
  inaccurate, and requiring unavailable infrastructure support. Finally, there
  are very few approaches that aim to make use of the elasticity and ease of
  control offered by cloud architectures. 
  Although cloud architectures provide a lot of elasticity, flexibility, and
  control, we are yet to see effective DDoS defenses and tolerance techniques
  that leverage the qualities of clouds to thwart such attacks. 
}


==> related.tex <==
%Traditionally, DDoS defense techniques are aimed at either {\em filtering} bad traffic
%or {\em authorizing} users before allocating resources. 
%Capability-based approaches~\cite{Xiaowei2008,Xiaowei2005,Parno2007}
%aim to authorize users by the means of
%cryptographic packet capabilities. Application servers issue capabilities
%typically during connection setup, and require the routers on the
%path between the clients and the servers to enforce their usage.
%Capabilities allow servers and routers to rate limit or blacklist users based
%on their observed behavior; detected bots will have their packets dropped as
%early as their gateway router.
%
%Filtering approaches rely on their ability to 
%differentiate between legitimate and attack traffic in the
%network~\cite{liu2008, liu2010},
%at the receiver~\cite{mahajan2002}, or at the Internet Service Provider
%(ISP)~\cite{fayaz2015}. The malicious traffic is then
%either dropped at the routers or redirected to specific parts of the protection
%mechanism for further
%analysis. 
%
%%% Need analysis of shortcomings of these approaches here!
%Both filtering and authorization techniques suffer from several drawbacks.
%First, they require changes
%to the core Internet routers along the paths between different endpoints.
%Additionally, some of the
%techniques require cooperation between ISPs, which is hard to achieve without
%proper incentives or government mandates.
%Furthermore, a crucial requirement for such techniques to work is their ability
%to differentiate between malicious and benign traffics.
%However, attackers often leverage IP spoofing, reflection attacks, and make use
%of very large botnets
%%(reaching up to millions of machines)
%of unsuspecting users as weapons for
%mounting DDoS attacks.
%This, therefore, makes the process of detecting malicious traffic and IP
%addresses intractable.
%
Among the end-to-end mitigations to SYN flood attacks, the SYN cache and TCP
SYN cookies are the most
common~\cite{rfc4987,lemon2002,cryptosyncookies}.
%%SYN cookies present a stateless method to combat server resource DoS attacks,
%specifically targeted
%%against SYN flooding attacks~\cite{lemon2002,cryptosyncookies}. SYN floods
%are
%attacks that target the three-way handshake of
%%TCP. 
%%Once a server receives a synchronize (SYN) packet froma potential client, it
%reserves a slot in
%%its queue for this client. In a SYN flood, the attackers overwhelm the server
%with a flood of SYN packets
%%and occupy the entire TCP backlog. Once that happens, the server discards new
%connection requests thus
%%hindering the new clients' connectivity and service availability. 
The SYN cache 
%attempts to reduce 
reduces the amount of memory needed to store state for
a half-open connection by delaying the
allocation of the full TCB state until the connection is established. Servers
implementing SYN caches instead maintain a
hash table for half-open connections that contains partial state
information and provides fast lookup and
insertion functions. SYN caches additionally impose limits on the number of
entries in the hash table as well as the
number of entries in each hash bucket. SYN cookies, on the other hand, operate
by eliminating 
%the source of the
%vulnerability in TCP implementations, 
the state reserved for half-open
connections in the TCB.
When SYN cookies are enabled, the server
encodes a new TCP connection's parameters as a cookie in the packet's initial
sequence number,
and refrains from allocating state for a new connection until the cookie is
again received from the client
and validated. 

The SYN cache aims to contain TCP SYN attacks
by reducing the amount of state maintained on the server for half-open
connections. Although efficient against
a single attacker (or a small botnet), SYN caches do no provide protection
against larger botnets
for which the attack rate can easily exceed the space allocated for the cache.
Once the cache is full, the server
will default to the same behavior it performed when its backlog limit is
reached, defeating the purpose for which
the cache is used.
Although SYN cookies eliminate the key target of the SYN flood attack (the TCP
backlog),
they do not provide protection against large botnets. Attackers in control of a
large number of
zombie machines with valid (non-spoofed) IP addresses can, without added
effort, overload the server's listen queue
with valid TCP requests at a rate that surpasses the server's ability to accept
them.
%% COMPLETED: \improvement{Aren't established connections removed from the
%% listen queue?}
%
By only tackling the problem on the server end, 
SYN cookies do not present a mechanism to strip the malicious actors from the
ability to conduct DoS attacks. Furthermore, it is not clear how SYN cookies can
be generalized to serve
as DoS protection schemes for different types of resource DoS attacks~\cite{wang2003}.
%(e.g. attacks against TLS connection
%setup)~\cite{wang2003}.

Laurie and Clayton~\cite{laurie2004proof} present an economic analysis to argue against the use of proof-of-work mechanisms 
to combat email spam. We agree with the authors' conclusion that computational puzzles do not possess ``magical'' properties
making them practical in every situation, and that proof-of-work must be properly analyzed before adoption; which is what 
we sought to achieve in this work. We argue that memory- and computational-resource exhaustion attacks are of a different nature
than spam emails. First, unlike spam, attacker benefits from DDoS attacks do not depend on the victim's response rate to every sent
packet; they are rather one-sided attacks. Second, DDoS attacks nowadays are mostly launched from compromised botnet machines and not
from specialized attacker hardware. Thus, beyond the initial compromise cost, launching an attack is virtually free for the attacker. 
We believe that our theoretical and experimental results showcase the merits of proof-of-work mechanisms in tolerating SYN and
connection floods.
%, and consist a step in the right direction towards the analysis and adoption of computational puzzles 
%for DDoS resilience. 
In fact, our work complements the security analysis 
performed in~\cite{liqun2009security,groza2014crypto,douglas2011stronger} with the required protocol engineering 
and design steps, allowing for a rich and improved understanding of client puzzles for DDoS resilience. 
\vspace{-0.5em}









==> titlepage.tex <==
%- Title page setup 
%\title{A Game-Theoretic Framework for Selecting Client Puzzle Difficulties}
\title{``Proof-of-Work" Proves to Work}
\subtitle{A Theoretical Formulation and Practical Implementation of TCP Puzzles for DDoS Tolerance}
%\title{DDoS Tolerance using TCP Client Puzzles \\ {\LARGE A Theoretical Formulation and Practical Implementation}}

%- Authors
%\author { }
%\author{Mohammad A. Noureddine}
%\affiliation{%
%  \institution{Coordinated Science Laboratory\\
%  University of Illinois at Urbana-Champaign}
%  \streetaddress{1308 W. Main St.}
%  \city{Urbana}
%  \state{Illinois}
%  \postcode{61801}}
%\email{nouredd2@illinois.edu}
%
%\author{William H. Sanders}
%\affiliation{%
%  \institution{Coordinated Science Laboratory\\
%  University of Illinois at Urbana-Champaign}
%  \streetaddress{1308 W. Main St.}
%  \city{Urbana}
%  \state{Illinois}
%  \postcode{61801}}
%\email{whs@illinois.edu}

